Data Generation Using Pass-phrase-dependent Deep Auto-encoders for Text-Dependent Speaker Verification

In this paper, we propose a novel method that trains pass-phrase specific deep neural network (PP-DNN) based auto-encoders for creating augmented data for text-dependent speaker verification (TD-SV). Each PP-DNN auto-encoder is trained using the utterances of a particular pass-phrase available in the target enrollment set with two methods: (i) transfer learning and (ii) training from scratch. Next, feature vectors of a given utterance are fed to the PP-DNNs and the output from each PP-DNN at frame-level is considered one new set of generated data. The generated data from each PP-DNN is then used for building a TD-SV system in contrast to the conventional method that considers only the evaluation data available. The proposed approach can be considered as the transformation of data to the pass-phrase specific space using a non-linear transformation learned by each PP-DNN. The method develops several TD-SV systems with the number equal to the number of PP-DNNs separately trained for each pass-phrases for the evaluation. Finally, the scores of the different TD-SV systems are fused for decision making. Experiments are conducted on the RedDots challenge 2016 database for TD-SV using short utterances. Results show that the proposed method improves the performance for both conventional cepstral feature and deep bottleneck feature using both Gaussian mixture model - universal background model (GMM-UBM) and i-vector framework.

==> References <==
@inproceedings{michelsanti2017conditional,
  title={{C}onditional Generative Adversarial Networks for Speech Enhancement and Noise-Robust Speaker Verification},
  author={Michelsanti, D. and Tan, Z.-H.},
  booktitle={Proc. of Interspeech},
  pages={2008--2012},
  year={2017}
}
@article{zeinali2019short,
  title={Short-duration Speaker Verification (SdSV) Challenge 2020: the Challenge Evaluation Plan},
  author={Zeinali, Hossein and Lee, Kong Aik and Alam, Jahangir and Burget, Lukas},
  journal={arXiv preprint arXiv:1912.06311},
  year={2019}
}

@Article{Mahalanobis36,
	author={P. C. Mahalanobis},
	title={{O}n the {G}eneralised {D}istance in {S}tatistics},
	journal={Proc. of the National Institute of Sciences of India},
        volume={2},
	pages={49-55},
	year={1936}
}


@Article{MacQueen67,
	author={J. MacQueen},
	title={{S}ome {M}ethods for {C}lassification and {A}nalysis of {M}ultivariate {O}bservations},
	journal={Proc. Fifth Berkeley Symp. on Math. Statist. and Prob. (Univ. of Calif. Press)},
	volume={1},
	pages={281-297},
	year={1967}
}

@Article{ross74,
	author={M. J. Ross and  H. L. Shaffer and A. Cohen and R. Freudberg and H. J.Manley},
	title={{A}verage {M}agnitude {D}ifference {F}unction {P}itch {E}xtractor},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={22},
	pages={353-362},
	year={1974}
}

@INPROCEEDINGS{Makhoul75,
	author = {J. Makhoul},
	title = {{L}inear {P}rediction: {A} {T}utorial {R}eview},
	booktitle = {Proceedings of the IEEE},
	volume={63},
	pages={561-580},
	year={1975}
}

@Article{Sambur76,
	author = {M. R. Sambur},
	title = {{S}peaker {R}ecognition using {O}rthogonal {L}inear {P}rediction},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={24},
	pages={283-289},
	year={1976}
}
	
@Article{Markel77,
	author = {J. D. Markel and B. T. Oshika and Jr. A. M. Gray},
	title = {{L}ong-term {F}eature {A}veraging for {S}peaker {R}ecognition},
        journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={25},
	pages={330-337},
	year={1977}
}

@Article{dempster77,
  author={A. Dempster and N. Laird and D. Rubin},
  title={{M}aximum {L}ikelihood from {I}ncomplete {D}ata via {EM} {A}lgorithm},
  journal={J. Roy. statist. Soc.},
  volume={39},
  pages={1-38},
  year={1977}
   }

@Article{Davis80,
	author={S. B. Davis and P. Mermelstein},
	title={{C}omparison of Parametric Representations for Monosyllabic Word Recognition in Continuously Spoken Sentences},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={28},
	pages={357-366},
	year={1980}
}

@Article{LINDE80,
	author={Y. Linde and A. Buzo and  R. M. GRAY},
        title={{A}n {A}lgorithm for {V}ector {Q}uantizer {D}esign},
	journal={IEEE Trans. Communications},
	volume={28},
	pages={84-94},
	year={1980}
}

@Article{Furui81,
	author={S. Furui},
	title={{C}epstral {A}nalysis {T}echnique for {A}utomatic {S}peaker {V}erification},
	journal={IEEE Trans. on  Acoust. Speech Signal Processing},
	volume={29},
	pages={254-272},
	year={1981}
}

@Article{Rabiner89,
	author={L. R. Rabiner},
	title={{A} {T}utorial on {H}idden {M}arkov {M}odels and {S}elected {A}pplications in {S}peech {R}ecognition},
	journal={Proc. of the IEEE},
	volume={77},
	pages={257-285},
	year={1989}
}



@Article{Hermansky90,
	author={H. Hermansky},
	 title={{P}erceptual Linear Predictive (PLP) Analysis of Speech},
	 journal={J. Acoust. Soc. Am.},
	 volume={87},
	 pages={1738-1752},
	 year={1990}
}

@Article{Higgin91,
author="A. Higgins and L. Bahler and J. Porter",
title="{S}peaker {V}erification using {R}andomized {P}hrase {P}rompting",
journal="Digital Signal Processing",
volume="1",
 pages="89-106",
year="1991"	 
}

@INPROCEEDINGS{reynolds91,
	author = {D. A. Reynolds and L. P. Heck},
	title = {{I}ntegration of {S}peaker and {S}peech {R}ecognition {S}ystems},
         booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {869-872},
	year = {1991}
}


@INPROCEEDINGS{Rosenberg92,
	author = {A. E. Rosenberg and J. DeLong and C\-H Lee and B\-H Jaung and F. K. Soong},
	title = {{T}he {U}se of {C}ohort {N}ormalized {S}cores for {S}peaker {V}erification},
	booktitle = { Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {599-602},
	year = {1992}
}

@Article{Hermanksy94,
       author = {H. Hermanksy and N. Morgan},
       title = {{R}ASTA Processing of Speech},
       journal={IEEE Trans. on Speech and Audio Processing},
       volume={2},
       pages={578-589},
       year={1994}
}

@Article{Gauvain94,
	author = {J.-L. Gauvain and C.-H. Lee},
	title = {{M}aximum a {P}osteriori {E}stimation for {M}ultivariate {G}aussian {M}ixture {O}bservations of {M}arkov {C}hains},
	journal={IEEE Trans. on Speech and Audio Processing},
	volume={2},
	pages={291-298},
	 year={1994}
}


@Article{reynold95,
  author="D. A. Reynolds",
  title="{S}peaker {I}dentification and {V}erification using {G}aussian {M}ixture {S}peaker {M}odels",
  journal="Speech Communication",
  volume="17",
  pages="91-108",
  year="1995"
}

@Article{Leggeter95,
author="C. Leggetter and P. Woodland",
title="{M}aximum {L}ikelihood {L}inear {R}egression for {S}peaker {A}daptation of {H}MMs",
journal="Computer Speech and Language",
volume="9",
pages="171-186",
year="1995"	
}
@Article{Vapnik95,
	author={C. Cortes and V. Vapnik},
	title={{S}upport {V}ector {N}etworks},
	journal={Machine Learning},
	volume={20},
	pages={273-297},
	year={1995}
}

@INPROCEEDINGS{Talkin95,
	author = {D. Talkin},
        title = {{A} {R}obust {A}lgorithm for {P}itch {T}racking ({RAPT})},
	booktitle = {in Speech coding and synthesis (Elsevier, ed.)},
	pages = {495-518},
        year = {1995}
}

@INPROCEEDINGS{leerose96,
 author = {Li Lee and Richard C. Rose},
 title = {{S}peaker {N}ormalization using {E}fficient {E}requency {W}arping {P}rocedures},
 booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages = {353-356},
 year = {1996}
}



@INPROCEEDINGS{Rosenberg96,
	 author = {A. E. Rosenberg and S. Parthasarathy},
	 title = {{S}peaker {b}ackground {m}odels for {c}onnected {d}igit {p}assword {s}peaker {V}erification},
	 booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {81-84},
	 year = {1996}
}




@INPROCEEDINGS{LHeck97,
	  author = {L. Heck and M. Weintraub},
	  title = {{H}andset-dependent {B}ackground {M}odels for {R}obust {T}ext-{I}ndependent {S}peaker {R}ecognition},
          booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	  pages = {1071-1074},
	  year = {1997}
}


@INPROCEEDINGS{DET97,
	   author = {A. Martin and G. Doddington and T. Kamm and M. Ordowskiand and M. Przybocki},
	   title = {{T}he DET Curve in Assessment of Detection Task Performance},
	   booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	   pages = {1895-1898},
	   year = {1997}
}  


@INPROCEEDINGS{Ariyaeeinia97,
	author= {A. M. Ariyaeeinia and P. Sivakumaran},
	title = {{A}nalysis and {C}omparison of {S}core {N}ormalization {M}ethods for {T}ext {D}ependent {S}peaker {V}erification},
	booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
        pages = {1379-1382},
	year = {1997}
}


@article{Lee-Rose98,
      author="L. Lee and R. Rose",
      title="{F}requency {W}arping {A}pproach  to {S}peaker {N}ormalization",
      journal="IEEE Trans. on Speech and Audio Processing",
      volume={6},
      pages={49-59},
      year={1998}
}



@INPROCEEDINGS{reycls98,
	author= {D. A. Reynolds and et. al},
	title = {{B}lind {C}lustering of {S}peech {U}tterances {B}ased on {S}peaker and {L}anguage {C}haracteristics},
	booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {3193-3196},
	year={1998}
}

@INPROCEEDINGS{Hermansky98,
	author={S. Van Vuuren and H. Hermansky},
	title={{O}n the {I}mportance of {C}omponents of the {M}odulation {S}pectrum for {S}peaker {V}erification},
        booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {3205-3208},
	year = {1998}
}


@Article{Pellom98,
    author={B. L. Pellom and J. H. L. Hansen},
    title={{A}n {E}fficient {S}coring {A}lgorithm for {G}aussian {M}ixture {M}odel {B}ased {S}peaker {I}dentification},
    journal={IEEE Signal Proc. Lett.},
    volume={5},
    pages={281-284},
    year={1998}
}

@Article{HLDA98,
	author= {N. Kumar and A.G. Andreou},
	title={{H}eteroscedastic {D}iscriminant {A}nalysis and {R}educed {R}ank {HMMs} for {I}mproved {S}peech {R}ecognition},
	journal={Speech Communication},
	volume={26},
	pages={283-297},
	year={1998}
}

@INPROCEEDINGS{Isobe99,
	author= {T. Isobe and J. Takahashi},
	title = {{A} {N}ew {C}ohort {N}ormalization using {L}ocal {A}coustic {I}nformation for {S}peaker {V}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
        pages = {841-844},
	year={1999}
}

@INPROCEEDINGS{McLaugn99,
     author={J. McLaughlin and D. A. Reynolds and T. Gleason},
     title={{A} {S}tudy of {C}omputation {S}peed-ups of the {GMM-UBM} {S}peaker {R}ecognition {S}ystem},
     booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
     pages={1215-1218},
     year={1999}
}

@INPROCEEDINGS{Markowitz99,
	author={J. Markowitz},
       title={{I}eri and {O}ggi {D}omani: {S}peaker {R}ecognition {Y}esterday, {T}oday and tomorrow},
       booktitle = {Proc. of COST250 Workshop on Speacker Recognition in Telephony},
       year={1999}
}


@INPROCEEDINGS{Auckenthaler1999,
author={R. Auckenthaler and  E. Parris and  M. Carey},
title={{I}mproving a {GMM} {S}peaker {V}erification {S}ystem by {P}honetic {W}eighting},
booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages={313-316},
 year={1999}
}


@Article{kuhn2000,
author="R. Kuhn and J.-C. Junqua and P. Nguyen and N. Niedzielski",
title="{R}apid {S}peaker {A}daptation in {E}igenvoice {S}pace",
journal="IEEE Trans. on Speech and Audio Processing",
volume="8 (6)",
pages="695-707",
year="2000"	
}	  

@Article{reynold00,
  author="D. A. Reynolds and T. F. Quatieri and R. B. Dunn",
  title="{S}peaker Verification using Adapted Gaussian Mixture Models",
  journal="Digital Signal Processing",
  volume="10",
  pages="19-41",
 year="2000"	  
}

@Article{Tnorm00,
 author="R. Auckenthaler and M. Carey and H. Lloyd-Thomas",
 title="{S}core {N}ormalization for {T}ext-{I}ndependent {S}peaker {V}erification {S}ystem",
 journal="Digital Signal Processing",
 Volume="10",
 pages="42-54",
 year="2000"
 }


@INPROCEEDINGS{Wagner00,
     author= {D. Tran and M. Wagner},
     title = {{A} {P}roposed {L}ikelihood {T}ransformation for {S}peaker {V}erification},
     booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
     pages = {1069-1072},
     year={2000}
}


@Article{kishore00,
  author="S. P. Kishore and B. Yegnanarayana",
  title="{S}peaker {V}erification: {M}inimizing the {C}hannel {E}ffects using {A}utoassociative {N}eural {N}etwork {M}odels",
  journal="ICASSP",
  year="2000",
  pages="1101-1104"
}



@INPROCEEDINGS{Heck00,
	author= {R. Teunen and B. Shahshahani and L. Heck},
	title = {{A} {M}odel-based {T}ransformational {A}pproach to {R}obust {S}peaker {R}ecognition},
	booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
        pages = {495-498},
        year={2000}
}

@INPROCEEDINGS{paliwal00,
	author= {B. Wildermoth and K. K. Paliwal},
	title = {{U}se of {V}oicing and {P}itch {I}nformation for {S}peaker {R}ecognition},
	booktitle = {Proc. 8th Australian Intern. Conf. Speech Science and Technology},
	pages = {324-328},
       year={2000}

}


@INPROCEEDINGS{Gadde2000,
	author= {V. R. R. Gadde},
	title = {{M}odeling {W}ord {D}uration},
        booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {601-604},
        year={2000}
}

@INPROCEEDINGS{Wan2000,
	author= {V. Wan and W. M. Campbell},
	title = {{S}upport {V}ector {M}achines for {S}peaker {V}erification and {I}dentification},
	booktitle = {Proc. IEEE Signal Processing Society Workshop Neural Networks},
	pages = {775-784},
	year={2000}
}


@INPROCEEDINGS{Doddington2001,
        author= {G. Doddington},
        title = {{S}peaker {R}ecognition {B}ased on {I}diolectal {D}ifferences {B}etween {S}peakers},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
        pages = {2521-2524},
        year={2001}
}  


@INPROCEEDINGS{Sturim01,
        author= {D. Sturim and D. A. Reynolds and E. Singer and J. P. Campbell},
        title = {{S}peaker {I}ndexing in {L}arge {A}udio {D}atabases using {A}nchor {M}odels},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {429-432},
        year={2001}
}

@INPROCEEDINGS{Auck01,
       author={R. Auckenthaler and J. S. Masion},
       title={{G}aussian {S}election {a}pplied to {T}ext-{I}ndependent {S}peaker {V}erification},
       booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={83-88},
       year={2001}
}

@INPROCEEDINGS{Pelecanos01,
       author={J. Pelecanos and S. Sridharan},
       title={{F}eature {W}arping for {R}obust {S}peaker {V}erification},
       booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={213-218},
       year= {2001}
}


@INPROCEEDINGS{Wang2001,
        author= {J. C. N. Wang and W. H. Tsai and L. S. Lee},
        title = {{E}igen-{MLLR} {C}oefficients as {N}ew {F}eature {P}arameters for {S}peaker {I}dentification},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {1385-1388},
        year={2001}
}


@INPROCEEDINGS{Kajarekar2001,
author= {S. Kajarekar and H. Hermansky},
title = {{S}peaker {V}erification {B}ased on {B}road {P}honetic {C}ategories},
booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
pages={201-206},
year={2001}
}

@INPROCEEDINGS{Glds_ker2002,
	author={W. M. Campbell},
	title={{G}eneralized {L}inear {D}iscriminant {S}equence {K}ernels for {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {161-164},
	year={2002}
}


@INPROCEEDINGS{ReynoldsFmap,
	author= {D.A. Reynolds},
	title = {{C}hannel {R}obust {S}peaker {V}erification via {F}eature {M}apping},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {6-10},
        year={2003}
}


@INPROCEEDINGS{Tkinnun03,
    author={T. Kinnunen and E. Karpov and P. Franti},
    title={{A} Speaker Pruning {A}lgorithm for {R}eal-{T}ime {S}peaker {I}dentification},
    booktitle = {Proc. Audio- and Video-Based Biometric Authentication},
    pages={639-646},
        year={2003}
}




@Article{nisteval04,
	author="{T}he {E}valuation {P}lan of NIST 2004 {S}peaker {R}ecognition {C}ampaign.
	http://www.itl.nist.gov/iad/mig//tests/sre/2004/SRE-04\_evalplan{-}v1a.pdf"
}

@INPROCEEDINGS{bonastre04,
        author = {J. F. Bonastre and N. Scheffer and C. Fredouille and D. Matrouf},
        title = {{N}IST'04 {S}peaker {R}ecognition {E}valuation {C}ampaign: {N}ew {LIA} {S}peaker {D}etection {P}lateform based on {ALIZE} {T}oolkit},
        booktitle = {Proc. of NIST 2004 Speaker Recognition Workshop},
        year = {2004},
}

@INPROCEEDINGS{Binma04,
	author = {B. Ma and H. Meng},
	title = {{E}nglish-{C}hinese {b}ilingual {t}ext-independent {s}peaker {v}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}

@INPROCEEDINGS{Leung04,
	author = {K. Y. Leung and M. W. Mak and S. Y. Kung},
	title = {{A}pplying {a}rticulatory {f}eatures to {t}elephone-based {s}peaker {v}erification},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}

@INPROCEEDINGS{Kwong04,
	author = {Q.Y. Hong and S. Kwong},
	title = {{D}iscriminative {t}raining for {s}peaker {i}dentification based on {m}aximum {m}odel {d}istance {a}lgorithm},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}


@ARTICLE {Bimbot04,
author = {F. Bimbot and J.-F. Bonastre and others},
journal = {EURASIP Journal on Applied Signal Processing},
pages = {430-451},
title = {A Tutorial on Text-Independent Speaker Verification},
volume = {4},
year = {2004}
}


@INPROCEEDINGS{Louradour05,
	author = {J. Louradour and K. Daoudi and R. Andre-Obrecht},
	title = {{D}iscriminative {P}ower of {T}ransient {F}rames in {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={613-616},
	year={2005}
}



@INPROCEEDINGS{Stolcke05,
	author= {A. Stolcke and L. Ferrer and S. Kajarekar and E. Shriberg and A. Venkataraman},
	title = {{MLLR} {T}ransforms as {F}eatures in {S}peaker {R}ecognition},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {2425-2428},
        year={2005}
}





@Article{kenny05,
author="P. Kenny",
title="{J}oint {F}actor {A}nalysis of {S}peaker and {S}ession {V}ariability : {T}heory and {A}lgorithms",
journal="Technical report CRIM-06/08-13  Montreal, CRIM",
year="2005"
}



@INPROCEEDINGS{AT_norm,
	author= {D. E. Sturim and D.A. Reynolds},
	title = {{S}peaker {A}daptive {C}ohort {S}election for {T}norm in {T}ext-independent {S}peaker {V}erification},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {741-744},
        year={2005}
}	


@INPROCEEDINGS{datadriven05,
	author= {M. Mason and R. Vogt and B. Baker and S. Sridharan},
	title = {{D}ata-{D}riven {C}lustering for {B}lind {F}eature {M}apping in {S}peaker {V}erification},
	booktitle = {Proc. of Interspeech},
         pages = {3109-3112},
        year={2005}
}


@INPROCEEDINGS{ZTnorm05,
	author= {R. Vogt and B. Baker and S. Sridharan},
	title = {{M}odeling {S}ession {V}ariability in {T}ext-{I}ndependent {S}peaker {V}erification},
	booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {3117-3120},
	year={2005}
}

@INPROCEEDINGS{Adami05,
	author= {André G. Adami},
        title = {{P}rosodic {M}odeling for {S}peaker {R}ecognition based on {S}ub-band {E}nergy {T}emporal {T}rajectories},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {189 - 192},
        year={2005}
}

@INPROCEEDINGS{NAP2005,
	author= {A. Solomonoff and W. M. Campbell and I. Boardman},
	title = {{A}dvances in {C}hannel {C}ompensation for {SVM} {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {629 - 632},
	year={2005}
}
@INPROCEEDINGS{Campbel_GMM_sup06,
author= {W. Campbell and D. Sturim and D. Reynolds and A. Solomonoff},
title = {{SVM} based {S}peaker {V}erification using a {GMM} {S}upervector {K}ernel and {NAP} {V}ariability {C}ompensation},
 booktitle = { Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages = {97-100},
 year={2006}
}

@INPROCEEDINGS{Goldberger05adistance,
author = {J. Goldberger and H. Aronowitz},
title = {{A} {D}istance {M}easure {B}etween {GMM}s {B}ased on the {U}nscented {T}ransform and its {A}pplication to {S}peaker {R}ecognition},
booktitle = {in Proc. of Interspeech},
pages = {1985-1989},
year = {2005}
}



@INPROCEEDINGS{krause06,
	author = {N. Krause and R. Gazit},
	title ={{SVM}-based {S}peaker {C}lassification in the {GMM} {M}odels {S}pace},
	booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
	year ={2006}
}


@INPROCEEDINGS{Noor06,
	  author = { E. Noor and H. Aronowitz},
	  title={{E}fficient {L}anguage {I}dentification using {A}nchor {M}odels and {S}upport {V}ector {M}achines},    
	  booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
	  year ={2006}
}



@inproceedings{Schwarz,
author = {Schwarz, P. and Matejka, P. and Cernocky, J.},
booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
pages = {325--328},
title = {{H}ierarchical {S}tructures of {N}eural {N}etworks for {P}honeme {R}ecognition},
year = {2006}
}


@INPROCEEDINGS{Binma06,
	author = {B. Ma and D. Zhu and R. Tong and H. Li},
	title={{S}peaker {C}luster {B}ased {GMM} {T}okenization for {S}peaker {R}ecognition},
	booktitle = {Proc. of Interspeech},
        year ={2006},
}


@INPROCEEDINGS{Hazen06,
  author="R. Woo and A. Park and T. J. Hazen",
  title="{T}he {MIT} {M}obile {D}evice {S}peaker {V}erification {C}orpus: {D}ata {C}ollection and {P}reliminary {E}xperiments",
  booktitle="Proc. of Odyssey Speaker and Language Recognition Workshop",
  pages="1-6",
  year="2006"
}


@Article{Campbell2006,
	author={W. M. Campbell and D. E. Sturim and D. A. Reynolds},
	title={{S}upport {V}ector {M}achines using {GMM} {S}upervectors for {S}peaker {V}erification},
	 journal={IEEE Signal Process. Lett.},
	 volume={13},
	 pages={308-311},
	 year={2006}
}


@Article{Mami06,
	author="Y. Mami and D. Charlet",
	title="{S}peaker {R}ecognition by {L}ocation in the {S}pace of {R}eference {S}peakers",
	journal="Speech Communication",
	volume="48",
	pages="127-141",
	year="2006"
}

@Article{Skosan06,
	author={M. Skosan and D. Mashao},
	title={{M}odified {S}egmental {H}istogram {E}qualization for {R}obust {S}peaker {V}erification},
	journal={Pattern Recogn. Lett.},
        volume={27},
        pages={479–486},
        year={2006}
}	


@INPROCEEDINGS{hatch06,
   author = {A. Hatch and S. Kajarekar and A. Stolcke},
   title={{W}ithin-{C}lass {C}ovariance {N}ormalization for {SVM}-{B}ased {S}peaker {R}ecognition},
   booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
   pages = {1471-1474},
   year ={2006}
}


@Article{htkbook,
  author="S. Young and D. Kershaw and J. Odell and V. Valtchev and P. Woodland and et al.",
  title="{HTK} {B}ook",
  journal={Copyright 2001-2006 Cambridge University Engineering Department}
   }


@Article{Castro2007,
      author="D. R. Castro and et. al",
      title="{S}peaker {V}erification using {S}peaker- and {T}est-dependent {F}ast {S}core {N}ormalization",
      journal="Pattern Recogn. Lett.",
      volume="28",
      pages="90-98",
      year="2007"
}

@INPROCEEDINGS{Charbuillet07,
	author={C. Charbuillet and B. Gas and M. Chetouani and J. L. Zarader},
	title={{C}omplementary {F}eatures for {S}peaker {V}erification based on {G}enetic {A}lgorithms},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={285-288},
	year = {2007}
}

@INPROCEEDINGS{Xugang07,
	author={X. Lu and J. Dang},
	 title={{P}hysiological {F}eature {E}xtraction for {T}ext {I}ndependent {S}peaker {I}dentification using {N}on-{U}niform {S}ub-band {P}rocessing},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={461-464},
        year = {2007}
}

@INPROCEEDINGS{Saeidi07,
	author={R. Saeidi and H. R. Sadegh Mohammadi and R. D. Rodman and T Kinnunen},
	title={{A} {N}ew {S}egmentation {A}lgorithm {C}ombined with {T}ransient {F}rames {P}ower for {T}ext {I}ndependent {S}peaker {V}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={305-308},
	year = {2007}
}
		
@INPROCEEDINGS{Tur2007,
	author={G. Tur and E. Shriberg and A. Stolcke and S. Kajarekar},
	title={{D}uration and {P}ronunciation {C}onditioned {L}exical {M}odeling for {S}peaker {S}erification},
        booktitle = {Proc. of Interspeech},
	pages={2049-2052},
	year = {2007}
}

@Article{HLDA_feat07,
	author={L. Burget and  P. Matejka and  O. Glembek and P. Schwarz and J. Cernocky},
        title = {{A}nalysis of {F}eature {E}xtraction and {C}hannel {C}ompensation in {GMM} {S}peaker {R}ecognition {S}ystem},
	journal={IEEE Trans. on Audio, Speech, Lang. Process.},
	volume={15},
	pages={1979-1986},
	year={2007}
}

@Article{fusion_2007,
	 author={N. Brummer and L. Burget and J. Cernocky and others},
	 title = {{F}usion of {H}eterogeneou {S}peaker {R}ecognition {S}ystems in the {STBU} {S}ubmission for the {NIST} {S}peaker {R}ecognition {E}valuation 2006},
	 journal={IEEE Trans. on Audio, Speech, and Lang. Process.},
	 volume={15},
	 pages={2072-2084},
	 year={2007}
}

@INPROCEEDINGS{Hazen97,
       author= {T. J. Hazen and J. R. Glass},
       title = {{A} {C}omparison of {N}ovel {T}echniques for {I}nstantaneous {S}peaker {A}daptation},
       booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
       pages = {2047-2050},
       year = {1997}
}


@INPROCEEDINGS{ferras-icassp08,
	author = {M. Ferras and  C. C. Leung and C. Barras and J. L. Gauvain},
        title = {{C}onstrained {MLLR} for {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {53-56},
	year = {2007}
}


	       


@inproceedings{akhil-interspeech2008,
      author = {P. T. Akhil and S. P. Rath and S. Umesh and D. R. Sanand},
      title = {{A} {C}omputationally {E}fficient {A}pproach to {W}arp {F}actor {E}stimation in {VTLN} Using {EM} {A}lgorithm and {S}ufficient {S}tatistics},
      booktitle = {Proc. of Interspeech},
      pages = {1713-1716},
      year = {2008}
}


@inproceedings{sanand-interspeech2008,
      author={D. R. Sanand and S. Umesh},
      title={{S}tudy of {J}acobian {C}ompensation Using {L}inear {T}ransformation of {C}onventional {MFCC} for {VTLN}},
      booktitle={Proc. of Interspeech},
      pages={1233-1236},
      year={2008}
}




@inproceedings{Yossi09,
	author = {Y. Bar-Yosef and Y. Bistritz},
        title = {{A}daptive {I}ndividual {B}ackground {M}odel for {S}peaker {V}erification},
        booktitle = {Proc. of Interspeech},
	pages = {1271-1274},
	year = {2009}
}	

@Article{Vraj09,
	author="V. R. Apsingekar and P. L. De Leon",
	title="{S}peaker {M}odel {C}lustering for {E}fficient {S}peaker {I}dentification in {L}arge {P}opulation {A}pplications",
	journal="IEEE Trans. on Speech and Language Processing",
	volume="17",
	pages="848-853",
	year="2009"
}


@article{kinnunen2010overview,
  title={{A}n Overview Of Text-independent Speaker Recognition: From Features To Supervectors},
  author={Kinnunen, T. and Li, H.},
  journal={Speech communication},
  volume={52},
  number={1},
  pages={12--40},
  year={2010}
 }



@inproceedings{achintya-odyssey2010,
	author= {A. K. Sarkar and S. Umesh},
	title= {{I}nvestigation of {S}peaker-{C}lustered {UBM}s based on {V}ocal {T}ract {L}engths and {MLLR} matrices for {S}peaker {V}erification},
	booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
	pages= {286-293},
	year = {2010}

}

@inproceedings{achintya-odyssey2010_spkid,
	      author= {A. K. Sarkar and S. Umesh and S. P. Rath},
	      title= {{C}omputationally {E}fficient {S}peaker {I}dentification for {L}arge {P}opulation {T}asks using {MLLR} and {S}ufficient {S}tatistics},
	      booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
	      pages= {7-11},
              year = {2010}
}


@inproceedings{Zhang-odyssey2010,
       author= {W. Q. Zhang and Y. Shan and J. Liu},
       title= {{M}ultiple {B}ackground {M}odels for {S}peaker {V}erification},
       booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={47-51},
       year = {2010}
}


@inproceedings{achintya-inter2010,
             author= {A. K. Sarkar and S. Umesh},
             title= {{F}ast {C}omputation of {S}peaker {C}haracterization {V}ector using {MLLR} and {S}ufficient {S}tatistics in {A}nchor {M}odel {F}ramework},
             booktitle = {Proc. of Interspeech},
	     pages={2738-2741},
	     year = {2010}
}


@inproceedings{achintya-icassp2011,
	        author= {A. K. Sarkar and S. Umesh},
	        title= {{U}se of {VTL}-wise {M}odels in {F}eature-{M}apping {F}ramework to {A}chieve {P}erformance of {M}ultiple-{B}ackground {M}odels in {S}peaker {V}erification},
	        booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
		pages={4552-4555},
	        year = {2011}

}

@inproceedings{SenoussaouiInterspch2011,
        author= {M. Senoussaoui and others},
        title= {{M}ixture of {PLDA} {M}odels {I}n {I}-{V}ector {S}pace {F}or {G}ender-{I}ndependent {S}peaker {R}ecognition},
        booktitle={Proc. of Interspeech},
        pages={25-28},
         year = {2011}
}


@Article{Deka_ieee2011,
       author= {N. Dehak and P. Kenny and R. Dehak and P. Ouellet and P. Dumouchel},
       title= {{F}ront-End Factor Analysis for Speaker Verification},
       journal={IEEE Trans. on Audio, Speech and Language Processing},
       volume={19},
       pages={788-798},
       year = {2011}
}

@inproceedings{Romero2011,
        author= {D. G. Romero and C. Y. Espy-Wilson},
        title= {{A}nalysis of i-vector {L}ength {N}ormalization in {S}peaker {R}ecognition {S}ystems},
        booktitle={Proc. of Interspeech},
        pages={249-252},
        year={2011}
}



@inproceedings{Kanagasundaram2011,
author={A. Kanagasundaram and R. Vogt and D. Dean and  S. Sridharan and M. Mason},
title= {i-vector based {S}peaker {R}ecognition on {S}hort {U}tterances},
booktitle={Proc. of Interspeech},
pages={2341-2344},
year={2011}
}

@inproceedings{Pierre-interspeech2012,
       author= {P. M. Bousquet and others},
       title= {{V}ariance-{S}pectra {B}ased {N}ormalization {F}or i-vector {S}tandard {A}nd {P}robabilistic {L}inear {D}iscriminant {A}nal
ysis},
       booktitle={Proc. of  Odyssey Speaker and Language Recognition Workshop},
       year={2012}
}

@inproceedings{Larcher2012,
author= {A. Larcher and K. A. Lee and  B. Ma and H. Li},
title= {{RSR2015}: {D}atabase for {T}ext-dependent {S}peaker {V}erification using {M}ultiple {P}ass-phrases},
booktitle={Proc. of Interspeech},
pages={1580-1583},
 year = {2012}
}

@inproceedings{achintya2012,
author={A. K. Sarkar and  D. Matrouf and P. M. Bousquet and J. F. Bonastre},
title= {{S}tudy of the Effect of i-vector Modeling on Short and Mismatch Utterance Duration for Speaker Verification},
booktitle={Proc. of Interspeech},
pages={2662-2665},
year={2012}
}




@inproceedings{Plchot2013,
author={O. Plchot and others},
title={{D}eveloping  a  {S}peaker  {I}dentification {S}ystem  for the {DARPA} {RATS} {P}roject},
booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
pages={ 6768-6772},
year={2013}
}





@inproceedings{Fu2014,
author={T. Fu and Y. Qian and Y. Liu and Kai Yu}, 
title= {{T}andem {D}eep {F}eatures for {T}ext-dependent {S}peaker {V}erification},
booktitle={Proc. of Interspeech},
pages={1327-1331},
year = {2014}
}

@inproceedings{Nicolas2014,
author={N. Scheffer and Y. Lei},
title= {{C}ontent {M}atching for {S}hort {D}uration {S}peaker {R}ecognition},
booktitle={Proc. of Interspeech},
pages={1317-1321},
year = {2014}
}

@inproceedings{Hagai2014,
author={H. Aronowitz and  A. Rendel},
title= {{D}omain {A}daptation for {T}ext {D}ependent {S}peaker {V}erification},
booktitle={Proc. of Interspeech},
pages={1337-1341},
year = {2014}
}


@Article{RSR2015,
author={A. Larcher and  K. A. Lee and  B. Ma and H. Li},
title= {{T}ext-dependent {S}peaker {V}erification: {C}lassifiers, {D}atabases and {RSR2015}},
journal={Speech Communucation},
volume={60},
pages={56-77},
year={2014}
}


@inproceedings{McLaren2015,
author={M. McLaren and Y. Lei and L. Ferrer},
title={{A}dvances {I}n {D}eep {N}eural {N}etwork {A}pproaches {T}o {S}peaker {R}ecognition},
booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year={2015}
}


@Article{Yuan2015,
author={Y. Liu and Y. Qian and N. Chen and T. Fu and Y. Zhang and K. Yu},
title= {{D}eep {F}eature for {T}ext-dependent {S}peaker {V}erification},
journal={Speech Communication},
volume={73},
pages={1-13},
year={2015}
}

@inproceedings{Delgado2016Asru,
author={H. Delgado and  M. Todisco and  M. Sahidullah and  A. K. Sarkar and N. Evans and  T. Kinnunen and  Z.-H. Tan},
title={{F}URTHER OPTIMISATIONS OF CONSTANT Q CEPSTRAL PROCESSING FOR INTEGRATED UTTERANCE AND TEXT-DEPENDENT SPEAKER VERIFICATION},
booktitle={Proc. of IEEE Spoken Language Technology Workshop (SLT)},
year={2016}
}

@misc{CNTK,
author= {A. Agarwal and others},
title= {{A}n {I}ntroduction to {C}omputational {N}etworks and the {C}omputational {N}etwork {T}oolkit},
year={2016},
howpublished ={https://www.microsoft.com/en-us/research/publication/an-introduction-to-computational-networks-and-the-computational-network-toolkit/}
}

@article{Tang2016,
author = {H. Tang},
title= {{S}equence {P}rediction with {N}eural {S}egmental {M}odels},
journal = {Ph.D. dissertation, Dept. Comput. Sci., Toyota Technological Inst. Chicago,
Chicago, IL, USA},
year =  {2017}
}


@inproceedings{yu2017adversarial,
  title={{A}dversarial {N}etwork {B}ottleneck {F}eatures {F}or {N}oise {R}obust {S}peaker {V}erification},
  author={Yu, H. and Tan, Z.-H. and Ma, Z. and Guo, J.},
  booktitle={Proc. of Interspeech},
  pages={1492--1496},
  year={2017}
}



@article{tang2017endtoend,
  title = {{E}nd-to-End {N}eural {S}egmental {M}odels {F}or {S}peech {R}ecognition},
  author = {H. Tang and L. Lu and K. Gimpel and K. Livescu and C. Dyer and N. A. Smith and S. Renals},
  year = {2017},
  pages={1254-1264},
  journal = {IEEE Journal of Selected Topics in Signal Processing},
  volume = {11}
}



@article{DBLP:journals/taslp/SarkarTTSG19,
  author    = {A. K. Sarkar and
               Z.-H. Tan and
               H. Tang and
               S. Shon and
               J. R. Glass},
  title     = {{T}ime-Contrastive Learning Based Deep Bottleneck Features for Text-Dependent Speaker Verification},
  journal   = {{IEEE/ACM} Trans. Audio, Speech {\&} Language Processing},
  volume    = {27},
  number    = {8},
  pages     = {1267--1279},
  year      = {2019}
}

@misc{xvector_recipe,
 title= {https://github.com/kaldi-asr/kaldi/tree/master/egs/sre16/v2}
 }
 
@inproceedings{conf/icassp/SnyderGSPK18,
  author    = {D. Snyder and
               D. Garcia{-}Romero and
               G. Sell and
               D. Povey and
               S. Khudanpur},
  title     = {{X}-Vectors: Robust DNN Embeddings for Speaker Recognition},
  booktitle = {Proc. of ICASSP},
  pages     = {5329--5333},
   year      = {2018}
}


@Article{alizetoolkit,
  title="http://lia.univ-avignon.fr/heberges/ALIZE/"
   }

@Article{mit_database,
  title="http://groups.csail.mit.edu/sls/mdsvc"
}

@Book{duda_hart_patt,
	  author = {R.O. Duda and P.E. Hart and D.G. Stork},
	  title  = {{P}attern {C}lassification},
	  publisher = {New York: John Wiley \& Sons},
	  year    = {2001}
}


@inproceedings{Timit,
author = {J. S. Garofolo and L. F. Lamel and W. M. Fisher and J. G. Fiscus and  D. S. Pallett and N. L. Dahlgren and V. Zue},
title = {{TIMIT} {A}coustic-{P}honetic {C}ontinuous {S}peech {C}orpus {LDC}93{S}1},
publisher = {Web Download. Philadelphia: Linguistic Data Consortium},
year={1993}
}


@inproceedings{noise_mix,
author= {A. Hannun and others},
title = {{D}eep Speech: Scaling Up End-to-End Speech recognition},
 booktitle= {in arXiv, 2014}
}


@article{Sarkar2017,
author = {A. K. Sarkar and Z.-H. Tan},
title ={{I}ncorporating {P}ass-phrase {D}ependent {B}ackground {M}odels for {T}ext-dependent {S}peaker {V}erification},
journal={ Computer speech \& Language},
volume={47},
year ={2018},
pages= {259-271}
}




@article{TanSD20,
  author    = {Z.-H. Tan and  A. K. Sarkar and N. Dehak},
  title     = {{rVAD}: An Unsupervised Segment-based Robust Voice Activity Detection Method},
  journal   = {Computer Speech \& Language},
  volume    = {59},
  pages     = {1--21},
  year      = {2020}

 } 



@article{Park_2019,
   title={{S}pecAugment: A Simple Data Augmentation Method for Automatic Speech Recognition},
    pages={2613--2617},
   author={Park, D. S. and others},
   year={2019},
   booktitle={Proc. of Interspeech}
}

@INPROCEEDINGS{Jaitly_vocaltract,
    author = {N. Jaitly and G. E. Hinton},
    title = {{V}ocal Tract Length Perturbation (VTLP) Improves Speech Recognition},
    booktitle = {Proc. of ICML},
    year = {2013}
}

@INPROCEEDINGS{Mauch2013,
author = {M. Mauch and S. Ewert},
title = {{T}he Audio Degradation Toolbox and its Application to Robustness Evaluation},
year = {2013},
booktitle = {Proc. of  ISMIR},
pages = {83-88}
}

@INPROCEEDINGS{Lasseck2018,
author = {M. Lasseck},
title= {{A}udio-based Bird Species Identification with Deep Convolutional Neural Networks},
booktitle = {In: Working Notes of CLEF 2018 (C{r}oss Lan{g}uage Evaluation Fo{r}um)}
}


@misc{Focal,
	author= {N. Brummer},
	title= {{F}oCal {T}oolkit},
       howpublished ={Available at http://sites.google.com/site/nikobrummer/focal}
}

@misc{Lnknet,
title= {http://www.ll.mit.edu/mission/communications/ist/lnknet/index.html}
}
@misc{RedDots,
title= {The RedDots Challenge: Towards Characterizing Speakers from Short Utterances},
howpublished ={https://sites.google.com/site/thereddotsproject/reddots-challenge}
}

@misc{SRE08,
title = {https://www.nist.gov/itl/iad/mig/2008-nist-speaker-recognition-evaluation-results}
}

@ARTICLE{7829341,
author={J. {Salamon} and J. P. {Bello}},
journal={IEEE Signal Processing Letters},
title={{D}eep Convolutional Neural Networks and Data Augmentation for Environmental Sound Classification},
year={2017},
volume={24}, 
number={3},
pages={279-283}
}


@ARTICLE{24792,  
author={F. L. {Bookstein}}, 
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},  
title={{P}rincipal Warps: Thin-plate Splines and the Decomposition of Deformations},
year={1989}, 
volume={11},
number={6}, 
pages={567-585}
}

@ARTICLE{Shorten2019,
author = {C. Shorten and T. M. Khoshgoftaar},
title = {{A} Survey on Image Data Augmentation for Deep Learning},
journal = {Journal of Big Data},
year ={2019}
}


@INPROCEEDINGS{ITU2005,
author = {ITU},
title = {{G.} 191: Software Tools for Speech and Audio Coding Standardization},
booketitle ={International Telecommunication Union},
year = {2005}

}



@INPROCEEDINGS{7528399,  
author={H. {Yu} and A. {Sarkar} and D. A. L. {Thomsen} and Z. {Tan} and Z. {Ma} and J. {Guo}},
booktitle={Proc. of SPLINE},  
title={{E}ffect of Multi-condition Training and Speech Enhancement Methods on Spoofing Detection},
year={2016}, 
pages={1-5}
}

@INPROCEEDINGS{I4U2013,
author = {R. Saeidi and others},
title = {{I4U} Ssubmission to NIST SRE 2012: A Large-scale Collaborative Effort for Noise-robust Speaker Verification},
pages= {1986-1990},
year ={2013},
Booktitle = {Proc. of Interspeech}
}

@INPROCEEDINGS{Stewart2010,
author = {R. Stewart and M. Sandler},
title = {{D}atabase of Omnidirectional and b-format Room Impulse Responses},
booktitle = {Proc. of ICASSP},
pages = {165-168},
year={2010}
}

@inproceedings{Hinton2012,
author = {G. Hinton and others},
title = {{D}eep {N}eural {N}etworks {F}or {A}coustic {M}odeling {I}n {S}peech {R}ecognition},
booktitle={IEEE Signal Process. Mag.},
pages={82-97},
year={2012}
}

@inproceedings{Kinnunen2016,
author={T. Kinnunen and others},
title={{U}tterance verification for text-dependent speaker recognition: a comparative assessment using the RedDots corpus},
booktitle={Proc. of Interspeech},
year={2016},
pages = {430-434}
}

 
@misc{tensorflow2015-whitepaper,
title={ {TensorFlow}: large-scale machine learning on heterogeneous systems},
url={https://www.tensorflow.org/},
note={Software available from tensorflow.org},
author={M. Abadi and
     others},
  year={2015}
}


@INPROCEEDINGS{Povey_ASRU2011,
         author = {Povey, D. and others},
         title = {{T}he Kaldi Speech Recognition Toolkit},
         booktitle = {Proc.   on Automatic Speech Recognition and Understanding (ASRU)},
           year = {2011},
      
}

@inproceedings{chung2020generative,
  title = {{G}enerative pre-training for speech with auto-regressive predictive coding},
  author = {Chung, Y.-A. and Glass, J.},
  booktitle = {Proc of ICASSP},
  year = {2020},
  pages={3497-3501}
}

@inproceedings{achintya_axriv2020,
title = {{D}ata augmentation enhanced speaker enrollment for text-dependent speaker verification},
author = {A. K. Sarkar and H. Sarma and  P. Dwivedi, Z.-H. Tan},
booktitle = {arXiv:2007.08004},
year = {2020}
}


@article{DBLP:journals/spl/SarkarDLB14,
  author    = {A. K. Sarkar and C. T. Do and V. B. Le and
               C. Barras},
  title     = {{C}ombination of cepstral and phonetically discriminative features for speaker verification},
  journal   = {{IEEE} Signal Process. Lett.},
  volume    = {21},
  number    = {9},
  pages     = {1040--1044},
  year      = {2014},
  }
  
 @InProceedings{Yim_2017_CVPR,
author = {Yim, J. and Joo, D. and Bae, J. and Kim, J.},
title = {{A} Gift From Knowledge Distillation: Fast Optimization, Network Minimization and Transfer Learning},
booktitle = {Proc. of CVPR},
year = {2017},
pages = {7130-7138}
} 

@INPROCEEDINGS{7472128,
  author={H. {Lim} and M. J. {Kim} and H. {Kim}},
  booktitle={Proc. of ICASSP}, 
  title={Cross-acoustic transfer learning for sound event classification}, 
  year={2016},
   pages={2504-2508}
  }
  
@INPROCEEDINGS{7953073,
  author={J. {Cui} and others},
  booktitle={Proc. of ICASSP}, 
  title={{K}nowledge distillation across ensembles of multilingual models for low-resource languages}, 
  year={2017},
  pages={4825-4829}
  }
  
  @INPROCEEDINGS{9054468,
  author={A. {Abad} and P. {Bell} and A. {Carmantini} and S. {Renais}},
  booktitle={Proc. of ICASSP}, 
  title={Cross Lingual Transfer Learning for Zero-Resource Domain Adaptation}, 
  year={2020},
   pages={6909-6913}
  }

@INPROCEEDINGS{Dong2015,
author ={D. Wang and  T. F. Zheng},
title ={{T}ransfer Learning for Speech and Language Processing},
booktitle={arXiv:1511.06066}
}

@ARTICLE{8700495,
  author={A. {Rahangdale} and S. {Raut}},
  journal={IEEE Access}, 
  title={{D}eep Neural Network Regularization for Feature Selection in Learning-to-Rank}, 
  year={2019},
  volume={7},
  pages={53988-54006}
  }

@INPROCEEDINGS{mocco_dict,
author={K. He and others},
title ={Momentum Contrast for Unsupervised Visual Representation Learning},
booktitle={arXiv:1911.05722},
year ={2020}
}
